Magazine Supply Optimization: a Case-study

Supply optimization is a complex and challenging task in the magazine retail industry because of the fixed inventory assumption, irregular sales patterns, and varying product and point-of-sale characteristics. We introduce AthenIA, an industrialized magazine supply optimization solution that plans the supply for over 20,000 points of sale in France. We modularize the supply planning process into a four-step pipeline: demand sensing, optimization, business rules, and operating. The core of the solution is a novel group conformalized quantile regression method that integrates domain expert insights, coupled with a supply optimization technique that balances the costs of out-of-stock against the costs of over-supply. AthenIA has proven to be a valuable tool for magazine publishers, particularly in the context of evolving economic and ecological challenges.

==> dummy.tex <==
\iffalse
\section{Ease of Use}

\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.
\fi

==> sections/context.tex <==
\section{Print magazine retail}
\label{sec:context}

The solution is built for a magazine publisher in France. The publisher owns more than 90 ``edutainment'' (education and entertainment) magazine titles of various periodicities: weekly, monthly, bimonthly, quarterly, and special editions. The magazines are sold in a regulated network of more than 22,000 points of sale (POS) in France. One specialty of the magazines retail is the fixed inventory. At a period of time, only one issue of each title is put up for sale. At the beginning of the sale period of each issue, a predefined number of copies of this issue is sent to a list of POSes of this issue. This list is called ``plate" in this paper. Replenishment rarely happens because the replenishment's costs usually surpass the benefits. At the end of the sale period, unsold copies will be returned back to the publisher (often to be destroyed). There are several layers of costs: production costs, registration costs\footnote{Registration costs are the costs of registering a title to the magazine retail network}, distribution costs, unsold costs\footnote{The costs related to the return and treatment---usually destroy of unsold copies}. The POSes also take a commission of the sold copies. In order to optimize the profit, for each issue, the publisher has to estimate which POSes to send magazine copies to (i.e. the plate of the issue) and the optimal amount of copies to send to each POS. With the decline of the print media industry and the rise of environmental awareness, this estimation has become vital, economically and ecologically. 

Let us denote $<m,i>$ issue $i$ of title $m$. Mathematically, the objective is a complex formula as follows:
\begin{equation}
\label{eq:obj_global}
\begin{aligned}
\max_{s^{j}_{m,i}} \quad & \sum_{j \in \mathbb{P}^{}_{m, i}} \left( z^{j}_{m,i}*{price}_{m, i} - {cost}^{j}_{m, i}(s^{j}_{m,i}, s_{m,i}, z^{j}_{m,i}) \right)\\
\textrm{s.t.} \quad & s^{j}_{m,i}, z^{j}_{m,i} \in \mathbb{Z}^{0+},\\
  & s_{m,i} \in \left[N_{total}-\Delta, N+\Delta \right].
\end{aligned}
\end{equation}

with $\mathbb{P}^{}_{m, i}$ denotes the plate of $<m,i>$, $s^{j}_{m,i}$ denotes the supply of $<m,i>$ for POS $j$ (\ie how many copies of $<m,i>$ sent to POS $j$), $\mathbb{Z}^{0+}$ denotes the set of non-negative integers,  $s_{m,i} \triangleq \sum_{j \in \mathbb{P}^{}_{m, i}} s^{j}_{m,i} $ denotes the total supply of $< m,i >$, $N_{total}$ denotes the total supply constrain of $<m,i>$ imposed by the publisher, $\Delta$ denotes the tolerance of the total supply constraint,  $z^{j}_{m,i}$ denotes the sales of $<m,i>$ of POS $j$ when it is supplied $s^{j}_{m,i}$ copies, ${price}_{m, i}$ denotes the price of $<m,i>$, and ${cost}^{j}_{m, i}(s^{j}_{m,i}, s_{m,i}, z^{j}_{m,i})$ denotes the costs and commission taken by POS $j$ when it is supplied $s^{j}_{m,i}$ of $s_{m,i}$ total copies, and it sells $z^{j}_{m,i}$ copies. 

In layman's terms, Eq. \eqref{eq:obj_global} means to \textit{``find the plate and the number of copies sent to each POS in this plate to maximize the profit of issue $i$ of title $m$, given the cost structure ${cost}^{j}_{m, i}$ and the total supply constraint $N \pm \Delta$''}. 

In Eq. \eqref{eq:obj_global}, ${price}_{m, i}, \mathbb{S}, N,$ and $\Delta$ are known. $\mathbb{P}^{}_{m, i}$ is provided by a business rule. The formula of ${cost}^{j}_{m, i}$ is also known. However, the value of ${cost}^{j}_{m, i}(s^{j}_{m,i}, s_{m,i}, z^{j}_{m,i})$ depends not only on $s^{j}_{m,i}$ and $z^{j}_{m,i}$ but also on the total supply $s_{m,i}$. Another complication of Eq. \eqref{eq:obj_global} is the sales $z^{j}_{m,i}$ depends on the supply  $s^{j}_{m,i}$. Note that $z^{j}_{m,i}$ denotes the sales, not the demand. Let us denote $d^{j}_{m,i} \in \mathbb{R}^{0+}$\footnote{Unlike $z^{j}_{m,i}$ which is a non-negative integer, we define $d^{j}_{m,i}$ as a non-negative real number.} the demand of $<m,i>$ at POS $j$. We have: 
\begin{equation}
\label{eq:sales_demand}
    z^{j}_{m,i} = \min(d^{j}_{m,i}, s^{j}_{m,i}).
\end{equation}

 When $s^{j}_{m,i} > z^{j}_{m,i}$, the sales is equal to the demand. However, when there is an out-of-stock (i.e. $s^{j}_{m,i} = z^{j}_{m,i}$), there is potentially an unobserved demand that was missing. We can measure only the sales, not the demand. Moreover, the demand also depends on the supply. Suppose that we send 4 copies to a POS and it sells 3. This does not imply that if we sent 10 copies to this POS, it would sell the same 3. This ``visibility effect" is common in retail \cite{gul_retail_2023, lu_developing_2015}. 



One of the key factors of the optimization in Eq. \eqref{eq:obj_global} is the estimation of the demand $d^{j}_{m,i}$, which would then give us the sales $z^{j}_{m,i}$ using Eq. \eqref{eq:sales_demand}. This estimation faces several other challenges: for each title, the content of one issue to another varies significantly, hence the demand. The demands are highly seasonal and highly impacted by public holidays. Some POSes can be partially closed during the sale period. For new titles, or when new POSes join the network, there are no historical data (the cold-starting problem). Another challenge is some issues are sold with ``extra-products" (a.k.a gift-on-purchase, they can be a toy model of a car, or a set of colored pencils, \etc.), and the demands are heavily impacted by these extra-products. For example, if an issue is sold with a toy model of a dinosaur, the sales are usually boosted 10\% in compared to normal. In this paper, for the sake of simplicity, we use the term ``product" for the package that is sold to consumers, either a copy of an issue if this issue is sold without extra-products, or a copy of an issue with the extra-product(s) if the issue is sold with extra-product(s).

% The optimal supply of an issue depends not only on the demand of this issue but also on some strategies and constraints of the publisher. For example, the publisher may want to over supply an issue a little to increase the visibility of the title. 





==> sections/introduction_og.tex <==
\section{Introduction}
\label{sec:introduction}

The print magazine has long been a staple in our culture, serving as a source of information, entertainment, and education. However, the rapid evolution of technology and digital media has profoundly transformed the media industry. In the last decades, there has been a \rvv{marked} shift in customer preferences toward digital platforms, which offer faster and more accessible content that appeals to the visual sensibilities of modern audiences. As newer generations increasingly favor instant online content over traditional print \rvv{sources}, print magazines are facing significant difficulties in maintaining both relevance and profitability. This ongoing shift has profound implications for print media companies, as they struggle to adapt to a landscape where digital media continues to gain domination. \rv{Moreover, the print magazine industry is confronting emerging sustainability challenges. Growing societal awareness of environmental impacts, shifting consumer preferences, rising production costs, and increasing sustainability-related taxes \cite{noauthor_definition_nodate, noauthor_plastics_nodate} have made sustainable practices within the industry essential.} 

In this context, the role of supply optimization becomes crucial, bearing significant impacts. On one hand, efficient supply helps increase profit by minimizing the losses due to out-of-stock (oos) and reducing the costs associated with excess supply. On the other hand, by curbing oversupply, the industry can mitigate its environmental footprint by reducing waste and the ecological ramifications of unsold print papers. 


\rv{However, magazine supply optimization presents significant challenges. In magazine retail, the inventory is fixed. At the beginning of the selling period of an issue of a title, a predefined number of copies is sent to a specific list of Points Of Sale (POSes), referred to as the ``plate" in this paper. Replenishment is rare because the costs generally outweigh the benefits. At the end of the selling period, unsold copies are returned to the publisher, often to be destroyed. There are several layers of costs: production costs, registration costs (the costs of registering a title to the magazine retail network), distribution costs, and unsold costs (costs related to the return and treatment-usually destruction-of unsold copies). The POSes also take commissions on the sold copies. To optimize the profit, the publisher must define which POSes to send magazine copies to (\ie, the plate of the issue) and estimate the optimal number of copies to send to each POS.
With the decline of the print media industry and the rise of environmental awareness, this estimation has become crucial, both economically and ecologically.
}



Let us denote $<m,i>$ issue $i$ of title $m$. Mathematically, the objective is a complex formula as follows:
\begin{equation}
\label{eq:obj_global}
\begin{aligned}
\max_{s^{j}_{m,i}} \quad & \sum_{j \in \mathbb{P}^{}_{m, i}} \left( z^{j}_{m,i}*{price}_{m, i} - {cost}^{j}_{m, i}(s^{j}_{m,i}, s_{m,i}, z^{j}_{m,i}) \right)\\
\textrm{s.t.} \quad & s^{j}_{m,i}, z^{j}_{m,i} \in \mathbb{Z}^{0+},\\
  & s_{m,i} \in \left[N_{total}-\Delta, N_{total}+\Delta \right].
\end{aligned}
\end{equation}
with 
\begin{itemize}
    \item $\mathbb{P}^{}_{m, i}$ denotes the plate of $<m,i>$,
    \item $s^{j}_{m,i}$ denotes the supply of $<m,i>$ for POS $j$ (\ie how many copies of $<m,i>$ sent to POS $j$),
    \item $\mathbb{Z}^{0+}$ denotes the set of non-negative integers, 
    \item $s_{m,i} \triangleq \sum_{j \in \mathbb{P}^{}_{m, i}} s^{j}_{m,i} $ denotes the total supply of $< m,i >$,
    \item $N_{total}$ denotes the total supply constraint of $<m,i>$, imposed by the publisher,
    \item $\Delta$ denotes the tolerance of the total supply constraint,
    \item $z^{j}_{m,i}$ denotes the sales of $<m,i>$ at POS $j$,
    \item ${price}_{m, i}$ denotes the price of $<m,i>$,
    \item ${cost}^{j}_{m, i}(s^{j}_{m,i}, s_{m,i}, z^{j}_{m,i})$ denotes the costs and commission taken by POS $j$ when it is supplied $s^{j}_{m,i}$ of $s_{m,i}$ total copies, and it sells $z^{j}_{m,i}$ copies.
\end{itemize}
\rv{In layman's terms, Eq. \eqref{eq:obj_global} means to \textit{``find the number of copies sent to each POS in plate $\mathbb{P}^{}_{m, i}$ to maximize the profit of issue $i$ of title $m$, given the cost structure ${cost}^{j}_{m, i}$ and the total supply constraint $N \pm \Delta$''}}. 

In Eq. \eqref{eq:obj_global}, ${price}_{m, i}, N_{total},$ and $\Delta$ are known. $\mathbb{P}^{}_{m, i}$ is provided by a set of business rules. The formula of ${cost}^{j}_{m, i}$ is also known. However, the value of ${cost}^{j}_{m, i}(s^{j}_{m,i}, s_{m,i}, z^{j}_{m,i})$ depends not only on $s^{j}_{m,i}$ and $z^{j}_{m,i}$ but also on the total supply $s_{m,i}$. Another difficulty of Eq. \eqref{eq:obj_global} is the sales $z^{j}_{m,i}$ depends on the supply  $s^{j}_{m,i}$. Note that $z^{j}_{m,i}$ denotes the sales, not the demand. Let us denote $d^{j}_{m,i} \in \mathbb{R}^{0+}$ the demand of $<m,i>$ at POS $j$. We have: 
\begin{equation}
\label{eq:sales_demand}
    z^{j}_{m,i} = \min(d^{j}_{m,i}, s^{j}_{m,i}).
\end{equation}
% \footnote{Unlike $z^{j}_{m,i}$ which is a non-negative integer, we define $d^{j}_{m,i}$ as a non-negative real number.}
When $s^{j}_{m,i} > z^{j}_{m,i}$, the sales are equal to the demand. However, when there is an out-of-stock (\ie $s^{j}_{m,i} = z^{j}_{m,i}$), there is potentially an unobserved demand that was missing. We can measure only the sales, not the actual demand. Moreover, the demand also depends on the supply. For instance, suppose that we send 4 copies to a POS and it sells 3. This does not imply that if we sent 10 copies to this POS, it would sell the same 3. This ``visibility effect" is common in retail \cite{gul_retail_2021, lu_developing_2015}. 

One of the key factors of the optimization in Eq. \eqref{eq:obj_global} is the estimation of the demand $d^{j}_{m,i}$, which in turn determines the sales $z^{j}_{m,i}$ using Eq. \eqref{eq:sales_demand}. This estimation faces several other challenges: for each title, the content of one issue to another varies significantly, hence the demand. The demands are highly seasonal and greatly influenced by public holidays. Some POSes may be partially closed during the selling period. For new titles or when new POSes join the network, there are no historical data, leading to a cold-starting problem. Another challenge arises when issues are sold with ``extra-products" (a.k.a gift-on-purchase, they can be a toy model of a car, or a set of colored pencils, \etc.), which can significantly impact the demand. For example, an issue sold with a toy dinosaur typically sees a 10\% sales increase compared to normal.  In this paper, for the sake of simplicity, we use the term ``product" for the package sold to consumers, whether it is a copy of an issue alone or a copy of an issue with extra-product(s).

% \begin{figure}
%   % \centering
%   \includegraphics[width=\linewidth]{figures/sales_histogram.png}
%   \centering
%   \caption[]{Histogram of a random subset\footnotemark \textrm{ } of the sales. The sales follow a typical long-tail distribution.} 
%   \label{fig:sales_histogram}
% \end{figure}

% \rvv{The supply optimization is challenging because of the high variability in the demand. As shown in Figure \ref{fig:sales_histogram}, \footnotetext{We can not provide the histogram of the full data because of confidentiality reasons. The right hand side of the histogram was also cropped.}most POSes sell only 0, 1 or 2 copies of most issues, while a few POSes sell dozens to hundreds of copies of high-demand issues. Because of the large number of POSes in each plate (from a few thousand to tens of thousands), small errors in estimation can accumulate across the plate, leading to substantial inefficiencies. The complexity of managing such a vast distribution network requires advanced methods that can handle the inherent variability and scale of magazine sales across numerous POSes.} 

\rvv{Because of the large number of POSes in each plate (from a few thousand to tens of thousands), small errors in the estimation of the demand can accumulate across the plate, leading to substantial inefficiencies. The complexity of managing such a vast distribution network requires advanced methods that can handle the inherent variability and scale of magazine sales across numerous POSes.} 
\rv{Additionally, a supply optimization solution must adhere to various business constraints, such as maintaining a consistent presence of the title in the retail network. Furthermore, it must be flexible enough to accommodate different business strategies and potentially last-minute changes.}

\rv{To address these challenges, we developed AthenIA---an industrialized magazine supply optimization solution. The solution is built for a magazine publisher in France. The publisher owns over 90 ``edutainment'' (education and entertainment) magazine titles, which vary in periodicity, including weekly, monthly, bimonthly, quarterly, and special editions. The magazines are sold in a highly regulated retail network of more than 22,000 points of sale. 
The key points of the solution are as follows:}
\begin{itemize}
    \item \rv{Standardized pipeline for supply optimization: we introduce a systematic yet flexible pipeline for supply optimization. This pipeline is both methodological and agile, enabling it to adapt to various scenarios and supply strategies. Its design allows for generalization to other sectors beyond magazine publishing.}
    \item \rv{Human-in-the-loop group conformalized quantile demand sensing: we introduce a group conformalized quantile demand sensing approach that enhances the integration of domain expert knowledge to model different nuances in the characteristics of the products.}
    \item  \rv{Novel optimization technique: we present a novel optimization technique that optimizes the profit under various constraints, given the estimated demand and the cost structure of the business.}
\end{itemize}

\rv{The paper is organized as follows: Section \ref{sec:solution} provides a detailed description of the solution, followed by an analysis of the results in Section \ref{sec:evaluation}. We outline the deployment details in Section \ref{sec:deployment}, and compare the solution with related work in Section \ref{sec:related_work}. Finally, Section \ref{sec:conclusion} concludes with a discussion regarding the impact of the solution and practical consideration.}

